Think Twice, Click Once: Enhancing GUI Grounding via Fast and Slow Systems

Humans can flexibly switch between different modes of thinking based on task complexity: from rapid intuitive judgments to in-depth analytical understanding. However, current Graphical User Interface (GUI) grounding systems which locate interface elements based on natural language instructions rely solely on immediate prediction without reasoning, struggling to understand complex interface layouts with nested structures and hierarchical relationships, limiting their effectiveness on complex interfaces. Inspired by human dual-system cognition, we present Focus, a novel GUI grounding framework that combines fast prediction with systematic analysis. The framework dynamically switches between rapid and deliberate processing through an adaptive system switching based on task complexity, optimizing both efficiency and accuracy. Focus decomposes grounding into progressive stages: interface summarization, visual focused analysis, and precise coordinate prediction. This structured decomposition enables systematic understanding of both interface layouts and visual relationships. Extensive experiments show that Focus achieves state-of-the-art performance using only 300K of the training data with a 2B parameter model compared to existing approaches. Focus demonstrates superior performance particularly in complex GUI scenarios, achieving 77.4% average accuracy on ScreenSpot and 13.3% on the more challenging ScreenSpot-Pro. Our analysis reveals the effectiveness of this dual-system approach while demonstrating its potential for improving complex GUI interaction scenarios.

==> tables/alpha_exp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[h]
% \centering
% \renewcommand\arraystretch{1.1}
% \tabcolsep=0.25cm
% {\fontsize{10pt}{12pt}\selectfont
% \begin{tabular}{cccccccc}
% \hline
% \multirow{2}{*}{$\alpha$ } & \multicolumn{2}{c}{Mobile}    & \multicolumn{2}{c}{Desktop}   & \multicolumn{2}{c}{Web}       & \multirow{2}{*}{Average} \\ \cline{2-7}
%                                        & Text          & Icon/Widget   & Text          & Icon/Widget   & Text          & Icon/Widget   &                          \\ \hline
% 0.0                                    & 87.1          & 73.8          & 77.2          & 61.5          & 78.3          & 61.9          & 73.3                     \\
% 0.2                                    & 88.3          & 75.1          & 78.4          & 62.8          & 79.5          & 63.2          & 74.6                     \\
% 0.4                                    & 89.2          & 76.8          & 79.6          & 63.9          & 80.4          & 64.8          & 75.8                     \\
% 0.6                                    & \textbf{90.1} & \textbf{78.2} & \textbf{80.9} & \textbf{65.0} & \textbf{81.7} & \textbf{68.5} & \textbf{77.4}            \\
% 0.8                                    & 89.7          & 77.5          & 80.2          & 64.3          & 81.2          & 65.3          & 76.4                     \\
% 1.0                                    & 86.5          & 74.9          & 76.9          & 61.8          & 77.5          & 62.9          & 73.4                     \\ \hline
% \end{tabular}
% \label{tab:alpha_exp}
% \caption{Impact of the scaling factor $\alpha$ on Focus's performance across different platforms and interaction modalities. The system achieves optimal performance at $\alpha$ = 0.6, balancing between fast grounding and deep cognitive processing.}
% \end{table*}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \begin{table*}[]
% \centering
% \renewcommand\arraystretch{1.1}
% {\fontsize{9pt}{12pt}\selectfont
% \begin{tabular}{ccccccccc}
% \hline
% \multirow{2}{*}{$\alpha$} & \multicolumn{2}{c}{Mobile}    & \multicolumn{2}{c}{Desktop}   & \multicolumn{2}{c}{Web}       & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Average\\ (acc)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Avg Time\\ (s)\end{tabular}} \\ \cline{2-7}
%                           & Text          & Icon/Widget   & Text          & Icon/Widget   & Text          & Icon/Widget   &                                                                          &                                                                         \\ \hline
% 0.0                       & 87.1          & 73.8          & 77.2          & 61.5          & 78.3          & 61.9          & 73.3                                                                     & 1.4                                                                     \\
% 0.2                       & 88.3          & 75.1          & 78.4          & 62.8          & 79.5          & 63.2          & 74.6                                                                     & 2.0                                                                     \\
% 0.4                       & 89.2          & 76.8          & 79.6          & 63.9          & 80.4          & 64.8          & 75.8                                                                     & 2.4                                                                     \\
% 0.6                       & \textbf{90.1} & \textbf{78.2} & \textbf{80.9} & \textbf{65.0} & \textbf{81.7} & \textbf{68.5} & \textbf{77.4}                                                            & 2.6                                                                     \\
% 0.8                       & 89.7          & 77.5          & 80.2          & 64.3          & 81.2          & 65.3          & 76.4                                                                     & 3.7                                                                     \\
% 1.0                       & 86.5          & 74.9          & 76.9          & 61.8          & 77.5          & 62.9          & 73.4                                                                     & 5.4                                                                     \\ \hline
% \end{tabular}
% \label{tab:alpha_exp}
% \caption{Impact of the scaling factor $\alpha$ on \textsc{FOCUS}'s performance and efficiency trade-off. The Fast/Slow Ratio indicates the percentage of samples processed by fast versus slow systems. Average Time represents the mean processing time per sample. At $\alpha$ = 0.6, \textsc{FOCUS} achieves optimal balance with fast and slow processing, resulting in an average processing time of 2.6s while maintaining the highest accuracy.}
% \end{table*}

\begin{table*}[]
\centering
\renewcommand\arraystretch{1.1}
{\fontsize{9pt}{12pt}\selectfont
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{Setting} & \multicolumn{2}{c}{Mobile}    & \multicolumn{2}{c}{Desktop}   & \multicolumn{2}{c}{Web}       & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Avg acc\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Avg Time (s)\end{tabular}} \\ \cline{2-7}
                          & Text          & Icon/Widget   & Text          & Icon/Widget   & Text          & Icon/Widget   &                                                                          &                                                                         \\ \hline
w/o $\alpha$              & 88.4          & 75.6          & 78.8          & 62.3          & 79.8          & 64.1          & 74.8                                                                     & 3.2                                                                     \\
0.0                       & 87.1          & 73.8          & 77.2          & 61.5          & 78.3          & 61.9          & 73.3                                                                     & 1.4                                                                     \\
0.2                       & 88.3          & 75.1          & 78.4          & 62.8          & 79.5          & 63.2          & 74.6                                                                     & 2.0                                                                     \\
0.4                       & 89.2          & 76.8          & 79.6          & 63.9          & 80.4          & 64.8          & 75.8                                                                     & 2.4                                                                     \\
0.6                       & \textbf{90.1} & \textbf{78.2} & \textbf{80.9} & \textbf{65.0} & \textbf{81.7} & \textbf{68.5} & \textbf{77.4}                                                            & 2.6                                                                     \\
0.8                       & 89.7          & 77.5          & 80.2          & 64.3          & 81.2          & 65.3          & 76.4                                                                     & 3.7                                                                     \\
1.0                       & 86.5          & 74.9          & 76.9          & 61.8          & 77.5          & 62.9          & 73.4                                                                     & 5.4                                                                     \\ \hline
\end{tabular}
}
\caption{Impact of the scaling factor $\alpha$ on \textsc{Focus}'s performance and efficiency trade-off. "w/o $\alpha$" represents the baseline without Adaptive System Switching, where the model automatically switchs between fast and slow grounding system without control. At $\alpha$ = 0.6, \textsc{Focus} achieves a +2.6\% accuracy improvement over the non-adaptive baseline while reducing average processing time by 0.6s, demonstrating the effectiveness of our adaptive switching mechanism in balancing accuracy and efficiency.}
\label{tab:alpha_exp}
\end{table*}

==> tables/dualsystem_activate.tex <==
\begin{table}[]
\centering
\renewcommand\arraystretch{1.1}
\tabcolsep=0.05cm
{\fontsize{7pt}{10pt}\selectfont
\begin{tabular}{cccc}
\hline
Element Type & Fast Grounding(\%) & Slow Grounding(\%) & Total Samples \\ \hline
Text         & 76.9\%             & 23.1\%             & 697           \\
Icon/Widget  & 56.3\%             & 43.7\%             & 575           \\
Overall      & 66.5\%             & 33.5\%             & 1272          \\ \hline
\end{tabular}
\caption{Distribution of system activation across different element types in \textbf{ScreenSpot}. Text elements predominantly trigger the fast system, while icon/widget elements more frequently activate the slow system, demonstrating \textsc{Focus}'s adaptive behavior.}
\label{tab:system_activation}
\end{table}
